Physics Informed Neural Networks for Two Dimensional Incompressible Thermal Convection Problems

Physics informed neural networks (PINNs) have drawn attention in recent years in engineering problems due to their effectiveness and ability to tackle the problems without generating complex meshes. PINNs use automatic differentiation to evaluate differential operators in conservation laws and hence do not need to have a discretization scheme. Using this ability, PINNs satisfy governing laws of physics in the loss function without any training data. In this work, we solve various incompressible thermal convection problems including real applications and problems with comparable numerical or analytical results. We first consider a channel problem with an analytical solution to show the accuracy of our network. Then, we solve a thermal convection problem in a closed enclosure in which the flow is only due to the temperature gradients on the boundaries. Lastly, we consider steady and unsteady partially blocked channel problems that resemble industrial applications to power electronics.

==> figures/tikz_fv_storage.tex <==
% \documentclass{article}
% % main document, called main.tex
% \usepackage{tikz}
% \usetikzlibrary{external}
% \tikzexternalize % activate!
% \begin{document}


% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: 
\path (0,400); %set diagram left start at 0, and has height of 400
%Flowchart: Connector [id:dp36334759955028506] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (194,183) .. controls (194,180.24) and (196.24,178) .. (199,178) .. controls (201.76,178) and (204,180.24) .. (204,183) .. controls (204,185.76) and (201.76,188) .. (199,188) .. controls (196.24,188) and (194,185.76) .. (194,183) -- cycle ;
%Flowchart: Connector [id:dp8653833555960755] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (269,227) .. controls (269,224.24) and (271.24,222) .. (274,222) .. controls (276.76,222) and (279,224.24) .. (279,227) .. controls (279,229.76) and (276.76,232) .. (274,232) .. controls (271.24,232) and (269,229.76) .. (269,227) -- cycle ;
%Flowchart: Connector [id:dp08526177209282815] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (119,227) .. controls (119,224.24) and (121.24,222) .. (124,222) .. controls (126.76,222) and (129,224.24) .. (129,227) .. controls (129,229.76) and (126.76,232) .. (124,232) .. controls (121.24,232) and (119,229.76) .. (119,227) -- cycle ;
%Flowchart: Connector [id:dp6874435430624763] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (194,97) .. controls (194,94.24) and (196.24,92) .. (199,92) .. controls (201.76,92) and (204,94.24) .. (204,97) .. controls (204,99.76) and (201.76,102) .. (199,102) .. controls (196.24,102) and (194,99.76) .. (194,97) -- cycle ;
%Straight Lines [id:da9940553029697292] 
\draw    (348,270) -- (48,270) ;
%Straight Lines [id:da5950697408123997] 
\draw    (199.62,10.19) -- (48,270) ;
%Straight Lines [id:da46866012450159666] 
\draw    (199.62,10.19) -- (348,270) ;
%Straight Lines [id:da9978103716213578] 
\draw    (123.81,140.1) -- (198,270) ;
%Straight Lines [id:da5433918254300527] 
\draw    (123.81,140.1) -- (273.81,140.1) ;
%Straight Lines [id:da8973321401800765] 
\draw    (273.81,140.1) -- (198,270) ;
%Shape: Rectangle [id:dp44333340219292294] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (343,265.5) -- (353,265.5) -- (353,274.5) -- (343,274.5) -- cycle ;
%Shape: Rectangle [id:dp776353397622314] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (194.62,5.69) -- (204.62,5.69) -- (204.62,14.69) -- (194.62,14.69) -- cycle ;
%Shape: Rectangle [id:dp05701645899113017] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (268.81,135.6) -- (278.81,135.6) -- (278.81,144.6) -- (268.81,144.6) -- cycle ;
%Shape: Rectangle [id:dp009972070653662346] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (118.81,135.6) -- (128.81,135.6) -- (128.81,144.6) -- (118.81,144.6) -- cycle ;
%Shape: Rectangle [id:dp5507449511947009] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (44,265.5) -- (54,265.5) -- (54,274.5) -- (44,274.5) -- cycle ;
%Shape: Rectangle [id:dp5807100659462046] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 125; green, 255; blue, 162 }  ,fill opacity=1 ] (193,265.5) -- (203,265.5) -- (203,274.5) -- (193,274.5) -- cycle ;


% Text Node
\draw (205,145) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\overline{\phi }_{i}^{0}$};
% Text Node
\draw (128,192) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\overline{\phi }_{i}^{1}$};
% Text Node
\draw (275,189) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\overline{\phi }_{i}^{2}$};
% Text Node
\draw (205,61) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\overline{\phi }_{i}^{3}$};
% Text Node
\draw (141,140) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle S_{i}^{0}$};
% Text Node
\draw (67,233) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle S_{i}^{1}$};
% Text Node
\draw (218,232) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle S_{i}^{2}$};
% Text Node
\draw (185,30) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle S_{i}^{3}$};


\end{tikzpicture}
% \end{document}
